Fundamental Limits on Latency in Transceiver Cache-Aided HetNets

Stringent mobile usage characteristics force wire- less networks to undergo a paradigm shift from conventional connection-centric to content-centric deployment. With respect to 5G, caching and heterogeneous networks (HetNet) are key technologies that will facilitate the evolution of highly content- centric networks by facilitating unified quality of service in terms of low-latency communication. In this paper, we study the impact of transceiver caching on the latency for a HetNet consisting of a single user, a receiver and one cache-assisted transceiver. We define an information-theoretic metric, the delivery time per bit (DTB), that captures the delivery latency. We establish coinciding lower and upper bounds on the DTB as a function of cache size and wireless channel parameters; thus, enabling a complete characterization of the DTB optimality of the network under study. As a result, we identify cache beneficial and non-beneficial channel regimes.

==> content/tikz_ldm.tex <==
%\input{tikzheader}

%name number of pipes; position (x,y);
\newcommand{\ldmnewuser}[3]{
\begin{scope}[pipedot/.style={draw, circle, inner sep=0pt, minimum size=0.3cm}]
\def\username{#1}
\def\numPipes{#2}
\def\distanceDots{0.6}
\coordinate (position\username) at #3;

\foreach \x in {1,...,\numPipes} {
	\pgfmathparse{-(\x-1)*\distanceDots}
	\node[pipedot] (node\x\username) at ($(0, \pgfmathresult)+(position\username)$) {};
}
\node[draw,fit=(node1\username) (node\numPipes\username)] (group\username) {};
\end{scope}
} 

%name of user1, name of user2, no of pipes, shifted levels 
\newcommand{\ldmconnectusers}[4]{
\foreach \x in {1,...,#3} {
	\pgfmathtruncatemacro\mymacro{(\x+#4)}
	\draw[->, thick] (node\x #1)--(node\mymacro #2) ;
}
} 



%\begin{document}

\begin{tikzpicture}

%\ldmnewuser{Alice}{6}{(0,0)}
\ldmnewuser{HeNB}{4}{(0,0)}
%\node[node distance=0.1cm, above=of groupAlice] {Alice};
\node[node distance=0.1cm, above=of groupHeNB] {HeNB};
%\node[node distance=0.2cm, left=of node1Alice] {$a\otimes b$};
\node[node distance=0.2cm, left=of node1HeNB] {$a_1\oplus b_3$};
% \node[node distance=0.2cm, left=of node2Alice] {$a\otimes b\otimes b$};

\ldmnewuser{eNB}{4}{(0,-5)}
\node[node distance=0.1cm, above=of groupeNB] {eNB};
\node[node distance=0.2cm, left=of node1eNB] {$b_1$};
\node[node distance=0.2cm, left=of node2eNB] {$b_2$};
\node[node distance=0.2cm, left=of node3eNB] {$b_3$};
\node[node distance=0.2cm, left=of node4eNB] {$a_2$};

%\ldmnewuser{Bob}{6}{(5,0)}
\ldmnewuser{fU}{4}{(5,0)}
%\node[node distance=0.1cm, above=of groupBob] {Bob};
\node[node distance=0.1cm, above=of groupfU] {$U_1$};
\node[node distance=0.2cm, right=of node3fU] {$a_1$};
\node[node distance=0.2cm, right=of node4fU] {$a_2$};

%\ldmnewuser{Eve}{6}{(5,-5)}
\ldmnewuser{sU}{4}{(5,-5)}
%\node[node distance=0.1cm, above=of groupEve] {Eve};
\node[node distance=0.1cm, above=of groupsU] {$U_2$};
\node[node distance=0.2cm, right=of node2sU] {$b_1$};
\node[node distance=0.2cm, right=of node3sU] {$b_2$};
\node[node distance=0.2cm, right=of node4sU] {$b_3$};

% Connect Tx and Rx

%\ldmconnectusers{Alice}{Bob}{4}{1}
\ldmconnectusers{HeNB}{fU}{1}{2}
%\ldmconnectusers{Alice}{Eve}{2}{3}
\ldmconnectusers{eNB}{fU}{4}{0}
\ldmconnectusers{eNB}{sU}{3}{1}

% Coloring and marking specific areas
\node[right=of node3sU.south, yshift=-0.2cm, xshift=12pt] (sU1) {}; 
\node[right=of node2sU.north, yshift=0.2cm, xshift=12pt] (sU2) {}; 
\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(sU1) -- (sU2) node [black,midway,xshift=8pt] {$n_{d2}-n_{d1}$};
\node[right=of node3fU.south, yshift=-0.2cm, xshift=12pt] (fU1) {}; 
\node[right=of node3fU.north, yshift=0.2cm, xshift=12pt] (fU2) {}; 
\draw[decorate,thick,decoration={brace,amplitude=2pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(fU1) -- (fU2) node [black,midway,xshift=20pt] {$n_{d1}+n_{d3}-n_{d2}$};
\node[right=of node4fU.south, yshift=-0.2cm, xshift=12pt] (fU3) {}; 
\node[right=of node4fU.north, yshift=0.2cm, xshift=12pt] (fU4) {}; 
\draw[decorate,thick,decoration={brace,amplitude=2pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(fU3) -- (fU4) node [black,midway,xshift=6pt] {$n_{d2}-n_{d3}$};

\begin{scope}[on background layer]
%\node[fill=blue!10,fit=(node1fU) (node2fU)] (groupfUd1) {};
\node[pattern=vertical lines, pattern color=black,fit=(node1HeNB) (node1HeNB)] (groupHeNBd1) {};
\node[pattern=horizontal lines, pattern color=red!80,fit=(node1HeNB) (node1HeNB)] (groupHeNBd2) {};
\node[pattern=north west lines, pattern color=black,fit=(node1eNB) (node2eNB)] (groupeNBd1) {};
\node[pattern=vertical lines, pattern color=black,fit=(node3eNB) (node3eNB)] (groupeNBd3) {};
\node[pattern=north west lines, pattern color=red!80,fit=(node4eNB) (node4eNB)] (groupeNBd3) {};
\node[pattern=north west lines, pattern color=black,fit=(node1fU) (node2fU)] (groupfUd1) {};
\node[pattern=horizontal lines, pattern color=red!80,fit=(node3fU) (node3fU)] (groupfUd3) {};
\node[pattern=north west lines, pattern color=red!80,fit=(node4fU) (node4fU)] (groupfUd3) {};
\node[pattern=north west lines, pattern color=black,fit=(node2sU) (node3sU)] (groupsUd1) {};
\node[pattern=vertical lines, pattern color=black,fit=(node4sU) (node4sU)] (groupsUd3) {};
%\fill[blue!20,rounded corners] (0,0) rectangle (7,7);
\end{scope}


%\node[right=of node5Bob.south, yshift=-0.2cm] (bobcurly1) {}; 
%\node[right=of node2Bob.north, yshift=0.2cm] (bobcurly2) {}; 
%\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
%(bobcurly1) -- (bobcurly2) node [black,midway] {$n_1$};
%
%\node[right=of node5Eve.south, yshift=-0.2cm] (evecurly1) {}; 
%\node[right=of node4Eve.north, yshift=0.2cm] (evecurly2) {}; 
%\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
%(evecurly1) -- (evecurly2) node [black,midway] {$n_2$};
%
%\node[right=of node3Eve.south, yshift=-0.2cm] (evecurly3) {}; 
%\node[right=of node2Eve.north, yshift=0.2cm] (evecurly4) {}; 
%\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
%(evecurly3) -- (evecurly4) node [black,midway,xshift=0.4cm] {$n_1-n_2$};
%
%
%
%\begin{scope}[on background layer]
%\node[fill=blue!10,fit=(node2Bob) (node5Bob)] (groupBobn1) {};
%\node[fill=blue!50,fit=(node2Eve) (node3Eve)] (groupEven1n2) {};
%%\fill[blue!20,rounded corners] (0,0) rectangle (7,7);
%\end{scope}


%\draw[->,red] (node5Bob.south)--(node1Eve.north) ;
\end{tikzpicture}

\begin{tikzpicture}

%\ldmnewuser{Alice}{6}{(0,0)}
\ldmnewuser{HeNB}{4}{(0,0)}
%\node[node distance=0.1cm, above=of groupAlice] {Alice};
\node[node distance=0.1cm, above=of groupHeNB] {HeNB};
%\node[node distance=0.2cm, left=of node1Alice] {$a\otimes b$};
\node[node distance=0.2cm, left=of node1HeNB] {$a_4\oplus b_5$};
% \node[node distance=0.2cm, left=of node2Alice] {$a\otimes b\otimes b$};

\ldmnewuser{eNB}{4}{(0,-5)}
\node[node distance=0.1cm, above=of groupeNB] {eNB};
\node[node distance=0.2cm, left=of node1eNB] {$b_4$};
\node[node distance=0.2cm, left=of node2eNB] {$a_3$};
\node[node distance=0.2cm, left=of node3eNB] {$b_5$};
\node[node distance=0.2cm, left=of node4eNB] {$a_5$};

%\ldmnewuser{Bob}{6}{(5,0)}
\ldmnewuser{fU}{4}{(5,0)}
%\node[node distance=0.1cm, above=of groupBob] {Bob};
\node[node distance=0.1cm, above=of groupfU] {$U_1$};
\node[node distance=0.2cm, right=of node2fU] {$a_3$};
\node[node distance=0.2cm, right=of node3fU] {$a_4$};
\node[node distance=0.2cm, right=of node4fU] {$a_5$};

%\ldmnewuser{Eve}{6}{(5,-5)}
\ldmnewuser{sU}{4}{(5,-5)}
%\node[node distance=0.1cm, above=of groupEve] {Eve};
\node[node distance=0.1cm, above=of groupsU] {$U_2$};
\node[node distance=0.2cm, right=of node2sU] {$b_4$};
\node[node distance=0.2cm, right=of node4sU] {$b_5$};

% Connect Tx and Rx

%\ldmconnectusers{Alice}{Bob}{4}{1}
\ldmconnectusers{HeNB}{fU}{1}{2}
%\ldmconnectusers{Alice}{Eve}{2}{3}
\ldmconnectusers{eNB}{fU}{4}{0}
\ldmconnectusers{eNB}{sU}{3}{1}

% Coloring and marking specific areas
\node[right=of node2sU.south, yshift=-0.2cm, xshift=12pt] (sU1) {}; 
\node[right=of node2sU.north, yshift=0.2cm, xshift=12pt] (sU2) {}; 
\draw[decorate,thick,decoration={brace,amplitude=2pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(sU1) -- (sU2) node [black,midway,xshift=6pt] {$n_{d2}-n_{d3}$};

\node[right=of node2fU.south, yshift=-0.2cm, xshift=12pt] (fU5) {}; 
\node[right=of node2fU.north, yshift=0.2cm, xshift=12pt] (fU6) {}; 
\draw[decorate,thick,decoration={brace,amplitude=2pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(fU5) -- (fU6) node [black,midway,xshift=6pt] {$n_{d3}-n_{d1}$};

\node[right=of node3fU.south, yshift=-0.2cm, xshift=12pt] (fU1) {}; 
\node[right=of node3fU.north, yshift=0.2cm, xshift=12pt] (fU2) {}; 
\draw[decorate,thick,decoration={brace,amplitude=2pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(fU1) -- (fU2) node [black,midway,xshift=20pt] {$n_{d1}+n_{d3}-n_{d2}$};

\node[right=of node4fU.south, yshift=-0.2cm, xshift=12pt] (fU3) {}; 
\node[right=of node4fU.north, yshift=0.2cm, xshift=12pt] (fU4) {}; 
\draw[decorate,thick,decoration={brace,amplitude=2pt,mirror,raise=-0.7cm},xshift=20pt, yshift=8pt]
(fU3) -- (fU4) node [black,midway,xshift=6pt] {$n_{d2}-n_{d3}$};


\begin{scope}[on background layer]
%\node[fill=blue!10,fit=(node1fU) (node2fU)] (groupfUd1) {};
\node[pattern=vertical lines, pattern color=black,fit=(node1HeNB) (node1HeNB)] (groupHeNBd1) {};
\node[pattern=horizontal lines, pattern color=red!80,fit=(node1HeNB) (node1HeNB)] (groupHeNBd2) {};

\node[pattern=north west lines, pattern color=black,fit=(node1eNB) (node1eNB)] (groupeNBd1) {};
\node[pattern=north east lines, pattern color=red!80,fit=(node2eNB) (node2eNB)] (groupeNBd1) {};
\node[pattern=vertical lines, pattern color=black,fit=(node3eNB) (node3eNB)] (groupeNBd3) {};
\node[pattern=north west lines, pattern color=red!80,fit=(node4eNB) (node4eNB)] (groupeNBd3) {};

\node[pattern=north west lines, pattern color=black,fit=(node1fU) (node1fU)] (groupfUd1) {};
\node[pattern=north east lines, pattern color=red!80,fit=(node2fU) (node2fU)] (groupfUd1) {};
\node[pattern=horizontal lines, pattern color=red!80,fit=(node3fU) (node3fU)] (groupfUd3) {};
\node[pattern=north west lines, pattern color=red!80,fit=(node4fU) (node4fU)] (groupfUd3) {};

\node[pattern=north west lines, pattern color=black,fit=(node2sU) (node2sU)] (groupsUd1) {};
\node[pattern=north west lines, pattern color=red!80,fit=(node3sU) (node3sU)] (groupsUd1) {};
\node[pattern=vertical lines, pattern color=black,fit=(node4sU) (node4sU)] (groupsUd3) {};
%\fill[blue!20,rounded corners] (0,0) rectangle (7,7);
\end{scope}





%\node[right=of node5Bob.south, yshift=-0.2cm] (bobcurly1) {}; 
%\node[right=of node2Bob.north, yshift=0.2cm] (bobcurly2) {}; 
%\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
%(bobcurly1) -- (bobcurly2) node [black,midway] {$n_1$};
%
%\node[right=of node5Eve.south, yshift=-0.2cm] (evecurly1) {}; 
%\node[right=of node4Eve.north, yshift=0.2cm] (evecurly2) {}; 
%\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
%(evecurly1) -- (evecurly2) node [black,midway] {$n_2$};
%
%\node[right=of node3Eve.south, yshift=-0.2cm] (evecurly3) {}; 
%\node[right=of node2Eve.north, yshift=0.2cm] (evecurly4) {}; 
%\draw[decorate,thick,decoration={brace,amplitude=5pt,mirror,raise=-0.7cm},yshift=0pt]
%(evecurly3) -- (evecurly4) node [black,midway,xshift=0.4cm] {$n_1-n_2$};
%
%
%
%\begin{scope}[on background layer]
%\node[fill=blue!10,fit=(node2Bob) (node5Bob)] (groupBobn1) {};
%\node[fill=blue!50,fit=(node2Eve) (node3Eve)] (groupEven1n2) {};
%%\fill[blue!20,rounded corners] (0,0) rectangle (7,7);
%\end{scope}


%\draw[->,red] (node5Bob.south)--(node1Eve.north) ;
\end{tikzpicture}


%\begin{tikzpicture}
%\coordinate (coordSourceupleft1) at (0,0);
%\coordinate (coordChannelupleft1) at (10,0);
%
%\node (reliableSourceBitsLeft) at (coordSourceupleft1) {};
%\node[right=of reliableSourceBitsLeft] (reliableSourceBitsRight) {};
%\node[node distance=1cm, below=of reliableSourceBitsLeft] (secureSourceBitsLeft) {};
%\node[node distance=1cm, below=of reliableSourceBitsRight] (secureSourceBitsRight) {};
%\node[node distance=0.1cm, left=of secureSourceBitsRight] (secureSourceBitsBlack) {};
%\node[node distance=1cm, below=of secureSourceBitsRight] (bottomSourceRight) {};
%\node[node distance=0.1cm, left=of secureSourceBitsLeft] {\parbox{2cm}{Secure source bits}};
%\node[node distance=0.1cm, right=of secureSourceBitsRight] {$m_2-m_1$};
%\node[node distance=0.1cm, left=of reliableSourceBitsLeft] {\parbox{2cm}{Reliable source bits}};
%\node[node distance=0.1cm, right=of reliableSourceBitsRight] {$m_1$};
%
%\draw [fill=yellow!20] (reliableSourceBitsLeft) rectangle (bottomSourceRight);
%\draw [fill=yellow!50] (secureSourceBitsLeft) rectangle (bottomSourceRight);
%\draw [fill=black] (secureSourceBitsBlack) rectangle (bottomSourceRight);
%
%
%\node (reliableChannelBitsLeft) at (coordChannelupleft1) {};
%\node[right=of reliableChannelBitsLeft] (reliableChannelBitsRight) {};
%\node[node distance=1cm, below=of reliableChannelBitsLeft] (secureChannelBitsLeft) {};
%\node[node distance=1cm, below=of reliableChannelBitsRight] (secureChannelBitsRight) {};
%\node[node distance=0.1cm, left=of secureChannelBitsRight] (secureChannelBitsBlack) {};
%\node[node distance=1cm, below=of secureChannelBitsRight] (bottomChannelRight) {};
%\node[node distance=0.1cm, left=of secureChannelBitsLeft] {\parbox{2cm}{Secure source bits}};
%\node[node distance=0.1cm, right=of secureChannelBitsRight] {$m_2-m_1$};
%\node[node distance=0.1cm, left=of reliableChannelBitsLeft] {\parbox{2cm}{Reliable source bits}};
%\node[node distance=0.1cm, right=of reliableChannelBitsRight] {$m_1$};
%
%\draw [fill=yellow!20] (reliableChannelBitsLeft) rectangle (bottomChannelRight);
%\draw [fill=yellow!50] (secureChannelBitsLeft) rectangle (bottomChannelRight);
%\draw [fill=black] (secureChannelBitsBlack) rectangle (bottomChannelRight);
%
%\end{tikzpicture}
%
%
%\tikzstyle{antenna} = [regular polygon,regular polygon sides=3, draw,shape
%border rotate=180,minimum size=0.2pt,scale=0.3]
%\tikzstyle{waves} = [snake=expanding waves, segment amplitude = 1.5cm, segment length = 0.3 cm,draw ]
%\begin{tikzpicture}
%	\coordinate (usercoord) at (0,0);
%	\node[rectangle,draw, minimum width=1cm, minimum height=1cm] (user) at (usercoord) {Tx};
%	\node[antenna] (userant1) at ($(user.west)+(-0.3cm,0.3cm)$) {};
%    \path[waves]  (userant1.west) -- ($(userant1.west)+(-1cm,0)$);
%    \draw (user) -| (userant1);
%          
%\end{tikzpicture}

%\end{document}

==> content/tikz_stacks.tex <==
%\input{tikzheader}

\edef\defaultpgflinewidth{\the\pgflinewidth}
%\newlength{\defaultpgflinewidth}
%\setlength{\defaultpgflinewidth}{0.1cm}

%Previous level name, new level name, level height, level description
\newcommand{\placeLevelOnTop}[4]{
\node[draw, fill=white, line width=\defaultpgflinewidth, rectangle, minimum width=1cm,minimum height=#3,inner sep=0pt] (#2) at ($(#1.north)+(0,#3*0.5-\defaultpgflinewidth*0.5)$) {#4}; 
}

%Previous level name, new level name, level height, level description
\newcommand{\placeLevelBelowBottom}[4]{
\node[draw, color=black!20, fill=white, line width=\defaultpgflinewidth, rectangle, minimum width=1cm,minimum height=#3,inner sep=0pt] (#2) at ($(#1.south)+(0,-#3*0.5+\defaultpgflinewidth*0.5)$) {#4}; 
}

\newlength{\mylabelwidth}
%Base coordinate, Level name, level label 
\newcommand{\addLevelLabel}[3]{
\settowidth{\mylabelwidth}{\pgfinterruptpicture #3 \endpgfinterruptpicture}
\node at ($(#2.north west -| #1)+(-0.2cm,-\defaultpgflinewidth*0.5)+(-\mylabelwidth*0.5,0)$) {#3};
\begin{pgfonlayer}{background}
\draw[dashed] ($(#2.north west -| #1)+(-0.1cm,-\defaultpgflinewidth*0.5)$) -- ($(#2.north west)+(0,-\defaultpgflinewidth*0.5)$);
\end{pgfonlayer}
}

%Lower Level name, Upper level name, brace label
\newcommand{\addBraceRight}[3]{
\draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
(#1.south east) -- (#2.north east) node [black,midway,xshift=0.8cm,rotate=90] {\footnotesize
#3};
}

%Level name, dim label
\newcommand{\addDimensioningRight}[2]{
\draw[dashed] ($(#1.north east)+(0,-\defaultpgflinewidth*0.5)$) -- ($(#1.north east)+(0.6cm,-\defaultpgflinewidth*0.5)$);
\draw[dashed] ($(#1.south east)+(0,\defaultpgflinewidth*0.5)$) -- ($(#1.south east)+(0.6cm,\defaultpgflinewidth*0.5)$);
\draw[thick,<->] ($(#1.north east)+(0.3cm,-\defaultpgflinewidth*0.5)$) -- node[right,fill=white,inner sep=0pt,xshift=0.1cm] {#2} ($(#1.south east)+(0.3cm,\defaultpgflinewidth*0.5)$);
}

%Level name, dim label
\newcommand{\addDimensioningLeft}[2]{
\draw[dashed] ($(#1.north west)+(0,-\defaultpgflinewidth*0.5)$) -- ($(#1.north west)+(-0.6cm,-\defaultpgflinewidth*0.5)$);
\draw[dashed] ($(#1.south west)+(0,\defaultpgflinewidth*0.5)$) -- ($(#1.south west)+(-0.6cm,\defaultpgflinewidth*0.5)$);
\draw[thick,<->] ($(#1.north west)+(-0.3cm,-\defaultpgflinewidth*0.5)$) -- node[left,fill=white,inner sep=0pt,xshift=-0.1cm] {#2} ($(#1.south west)+(-0.3cm,\defaultpgflinewidth*0.5)$);
}



%\begin{document}

\begin{tikzpicture}

[
%
]
\coordinate (txOneY) at (0,0);
\coordinate (txTwoY) at ($(txOneY)+(1.5,0)$);
\coordinate (baseLeft) at ($(txOneY)+(-0.75cm,0)$);
\coordinate (txOneZ) at ($(txTwoY)+(2,0)$);
\coordinate (txTwoZ) at ($(txOneZ)+(1.5,0)$);

\node (ytx1) at ($(txOneY)+(0,-0.5)$) {Tx1};
\node (ytx2) at ($(txTwoY)+(0,-0.5)$) {Tx2};
\node  at ($(txOneY)!0.5!(txTwoY) + (0,-1)$) {$\textbf{Rx2}$};
\node (ztx1) at ($(txOneZ)+(0,-0.5)$) {Tx1};
\node (ztx2) at ($(txTwoZ)+(0,-0.5)$) {Tx2};
\node  at ($(txOneZ)!0.5!(txTwoZ) + (0,-1)$) {$\textbf{Rx1}$};

\placeLevelOnTop{txOneY}{d1}{0.5cm}{${D}_1$}
\placeLevelOnTop{d1}{c1}{1cm}{${C}_1$}
\placeLevelOnTop{c1}{b1}{0.5cm}{${B}_1$}

\placeLevelOnTop{txTwoY}{b2}{0.5cm}{${B}_2$}

\placeLevelOnTop{txOneZ}{d1}{0.5cm}{${B}_1$}

\placeLevelOnTop{txTwoZ}{d2z}{0.5cm}{${D}_2$}
\placeLevelOnTop{d2z}{c2z}{1cm}{${C}_2$}
\placeLevelOnTop{c2z}{b2z}{0.5cm}{${B}_2$}
\addLevelLabel{baseLeft}{c2z}{$2n_d-n_c$}
\addLevelLabel{baseLeft}{d2z}{$n_d$}
\addLevelLabel{baseLeft}{b2z}{$n_c$}

\addDimensioningRight{c2z}{$l_1$}


\draw[thick] ($(baseLeft)+(0,-\defaultpgflinewidth*0.5)$) -- ($(txTwoY)+(0.75cm,-\defaultpgflinewidth*0.5)$);
\draw[thick] ($(txOneZ)+(-0.75,-\defaultpgflinewidth*0.5)$) -- ($(txTwoZ)+(0.75cm,-\defaultpgflinewidth*0.5)$);

\end{tikzpicture}




%\end{document}

==> content/tikz_stuff.tex <==
\usepackage{ellipsis}
\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathreplacing,decorations.markings,shapes.geometric}
\tikzset{naming/.style={align=center,font=\small}}
\tikzset{antenna/.style={insert path={-- coordinate (ant#1) ++(0,0.25) -- +(135:0.25) + (0,0) -- +(45:0.25)}}}
%\tikzset{station/.style={naming,draw,shape=dart,shape border rotate=90, minimum width=10mm, minimum height=10mm,outer sep=0pt,inner sep=3pt}}
\tikzset{station/.style={naming,draw,shape=dart,minimum width=10mm, minimum height=10mm,outer sep=0pt,inner sep=3pt}}
%\tikzset{mobile/.style={naming,draw,shape=rectangle,minimum width=15mm,minimum height=7.5mm, outer sep=0pt,inner sep=3pt}}
\tikzset{mobile/.style={naming,draw,shape=rectangle,minimum width=12mm,minimum height=6mm, outer sep=0pt,inner sep=3pt}}
\tikzset{radiation/.style={{decorate,decoration={expanding waves,angle=90,segment length=4pt}}}}

\newcommand{\MUE}[1]{%
\begin{tikzpicture}[every node/.append style={rectangle,minimum width=0pt}]
\node [mobile,label={[inner ysep=+.3333em]\dots}] (box) {#1};

%\node [mobile] (box) {#1};
%\node at ($(ant1)!0.5!(ant2)$) {\dots};

\draw ([xshift=.25cm] box.south west) circle (4pt)
      ([xshift=-.25cm]box.south east) circle (4pt);

\fill ([xshift=.25cm] box.south west) circle (1pt)
      ([xshift=-.25cm]box.south east) circle (1pt);

\draw ([xshift=.25cm] box.north west) [antenna=1];
\draw ([xshift=-.25cm]box.north east) [antenna=2];
\end{tikzpicture}
}

\newcommand{\UE}[1]{%
\begin{tikzpicture}[every node/.append style={rectangle,minimum width=0pt}]
\node[mobile] (box) {#1};

\draw ([xshift=.25cm] box.south west) circle (4pt)
      ([xshift=-.25cm]box.south east) circle (4pt);

\fill ([xshift=.25cm] box.south west) circle (1pt)
      ([xshift=-.25cm]box.south east) circle (1pt);

\draw (box.north) [antenna=1];
\end{tikzpicture}
}

\newcommand{\MBS}[1]{%
\begin{tikzpicture}
\node[station] (base) {#1};

%\draw[line join=bevel] (base.110) -- (base.70) -- (base.north west) -- (base.north east) -- cycle;
\draw[line join=bevel] (base.100) -- (base.80) -- (base.110) -- (base.70) -- (base.north west) -- (base.north east);
\draw[line join=bevel] (base.100) -- (base.70) (base.110) -- (base.north east);

% original yshift=.8pt
%\draw[line cap=rect] ([xshift=.5cm,yshift=.3pt] base.north) [antenna=1];
%\draw[line cap=rect] ([yshift=.3pt]ant1 |- base.north) -- node[above,shape=rectangle,inner ysep=+.3333em]{\dots} ([xshift=-.5cm,yshift=.3pt]base.north) [antenna=2];
\draw[line cap=rect] ([xshift=-.1768cm,yshift=.6pt]base.north -| base.right tail) [antenna=1];
\draw[line cap=rect] ([yshift=.6pt]ant1 |- base.north) -- node[above,shape=rectangle,inner ysep=+.3333em]{\dots} ([xshift=.1768cm,yshift=.6pt]base.north -| base.left tail) [antenna=2];

%\draw[line cap=rect] ([yshift=.3pt]ant1 |- base.north) -- ([xshift=-.5cm,yshift=.3pt]base.north) [antenna=2];
%\node at ($(ant1)!0.5!(ant2)$) {\dots};
\end{tikzpicture}
}

\newcommand{\BS}[1]{%
\begin{tikzpicture}
\node[station] (base) {#1};

%\draw[line join=bevel] (base.110) -- (base.70) -- (base.north west) -- (base.north east) -- cycle;
\draw[line join=bevel] (base.100) -- (base.80) -- (base.110) -- (base.70) -- (base.north west) -- (base.north east);
\draw[line join=bevel] (base.100) -- (base.70) (base.110) -- (base.north east);

% original yshift=.8pt
\draw[line cap=rect] ([yshift=0pt]base.north) [antenna=1];
\end{tikzpicture}
}

==> content/tikzlibrarytikzmark.code.tex <==
%%
%% This is file `tikzlibrarytikzmark.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tikzmark.dtx  (with options: `tikzlibrary')
%% ----------------------------------------------------------------
%% tikzmark --- remembering absolute positioning with TikZ.
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\tikzset{%
  remember picture with id/.style={%
    remember picture,
    overlay,
    save picture id=#1,
  },
  every picture/.append style={%
    execute at end picture={%
      \ifpgfrememberpicturepositiononpage%
      \edef\pgf@temp{%
        \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\thepage}}}%
      \pgf@temp
      \fi%
    },
  },
  save picture id/.code={%
      \protected@write\pgfutil@auxout{}{%
        \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
  },
  if picture id/.code args={#1#2#3}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#3}%
    }{
      \pgfkeysalso{#2}%
    }
  },
  next page/.is choice,
  next page vector/.initial={\pgfqpoint{0pt}{0pt}},
  next page/below/.style={%
    next page vector={\pgfqpoint{0pt}{-\the\paperheight}}%
  },
  next page/above/.style={%
    next page vector={\pgfqpoint{0pt}{\the\paperheight}}%
  },
  next page/left/.style={%
    next page vector={\pgfqpoint{-\the\paperwidth}{0pt}}%
  },
  next page/right/.style={%
    next page vector={\pgfqpoint{\the\paperwidth}{0pt}}%
  },
  next page/ignore/.style={%
    next page vector={\pgfqpoint{0pt}{0pt}}%
  },
  tikzmark prefix/.initial=,%
  tikzmark suffix/.initial=,%
}
\def\tikzmark@pp@name#1{\csname pgfk@/tikz/tikzmark prefix\endcsname#1\csname pgfk@/tikz/tikzmark suffix\endcsname}%
\def\savepointas#1#2#3#4{%
  \expandafter\gdef\csname save@pt@#1\endcsname{#2}%
  \expandafter\gdef\csname save@pt@#1@offset\endcsname{\pgfqpoint{#3}{#4}}%
}
\def\savepicturepage#1#2{%
  \expandafter\gdef\csname save@pg@#1\endcsname{#2}%
}
\def\tmk@labeldef#1,#2\@nil{%
  \edef\tmk@label{\tikzmark@pp@name{#1}}%
  \def\tmk@def{#2}%
}
\tikzdeclarecoordinatesystem{pic}{%
  \pgfutil@in@,{#1}%
  \ifpgfutil@in@%
    \tmk@labeldef#1\@nil
  \else
    \tmk@labeldef#1,(0pt,0pt)\@nil
  \fi
  \@ifundefined{save@pt@\tmk@label}{%
    \tikz@scan@one@point\pgfutil@firstofone\tmk@def
  }{%
      \pgfsys@getposition{\csname save@pt@\tmk@label\endcsname}\save@orig@pic%
      \pgfsys@getposition{\pgfpictureid}\save@this@pic%
      \pgf@process{\pgfpointorigin\save@this@pic}%
      \pgf@xa=\pgf@x
      \pgf@ya=\pgf@y
      \pgf@process{\pgfpointorigin\save@orig@pic}%
      \advance\pgf@x by -\pgf@xa
      \advance\pgf@y by -\pgf@ya
      \pgf@xa=\pgf@x
      \pgf@ya=\pgf@y
    \pgf@process{\pgfpointorigin\csname save@pt@\tmk@label @offset\endcsname}%
    \advance\pgf@xa by \pgf@x
    \advance\pgf@ya by \pgf@y
      \@ifundefined{save@pg@\csname save@pt@\tmk@label\endcsname}{}{%
        \@ifundefined{save@pg@\pgfpictureid}{}{%
          \pgfkeysvalueof{/tikz/next page vector}%
          \advance \pgf@xa by \csname save@pg@\csname save@pt@\tmk@label\endcsname\endcsname\pgf@x\relax
\advance \pgf@ya by \csname save@pg@\csname save@pt@\tmk@label\endcsname\endcsname\pgf@y\relax
          \advance \pgf@xa by -\csname save@pg@\pgfpictureid\endcsname\pgf@x\relax
\advance \pgf@ya by -\csname save@pg@\pgfpictureid\endcsname\pgf@y\relax
        }%
      }%
      \pgf@x=\pgf@xa
      \pgf@y=\pgf@ya
    \pgftransforminvert
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    }%
  }
\begingroup
\catcode`\;=\active
\gdef\tikzmark@active#1#2{%
\tikz[remember picture with id=#2] #1;}
\endgroup
\def\tikzmark@nonactive#1#2{%
\tikz[remember picture with id=#2] #1;}
\newcommand\tikzmark@outside[2][]{%
  \ifnum\catcode`\;=\active
   \let\tikzmark@next=\tikzmark@active
  \else
   \let\tikzmark@next=\tikzmark@nonactive
  \fi
  \tikzmark@next{#1}{#2}%
}
\def\tikzmark@inside#1#2{%
  \tikzset{remember picture}%
  \tikz@scan@one@point\pgfutil@firstofone#2\relax
  \protected@write\pgfutil@auxout{}{%
    \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{\the\pgf@x pt}{\the\pgf@y pt}}%
}
\def\tikzmark{%
  \ifx\pgfpictureid\@undefined
  \let\tikzmark@next=\tikzmark@outside
  \else
  \let\tikzmark@next=\tikzmark@inside
  \fi
  \tikzmark@next%
}
\newcommand\pgfmark[1]{%
    \bgroup
    \global\advance\pgf@picture@serial@count by1\relax%
    \edef\pgfpictureid{pgfid\the\pgf@picture@serial@count}%
      \pgfsys@markposition{\pgfpictureid}%
    \edef\pgf@temp{%
      \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\thepage}}}%
    \pgf@temp
    \protected@write\pgfutil@auxout{}{%
      \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
    \egroup
  }
\@ifclassloaded{beamer}{
  \renewcommand<>{\tikzmark}[2][]{\only#3{\beameroriginal{\tikzmark}[{#1}]{#2}}}
}{}
\@ifclassloaded{beamer}{
  \renewcommand<>{\pgfmark}[1]{\only#2{\beameroriginal{\pgfmark}{#1}}}
}{}
\@ifclassloaded{beamer}{
  \tikzset{
    tikzmark suffix=-\the\beamer@slideinframe
  }
}{}
\newcommand\iftikzmark[3]{%
    \@ifundefined{save@pt@#1}{%
      #3%
    }{%
      #2%
    }%
  }%
\newcommand\subnode[3][]{%
  \begingroup
  \pgfmark{#2}%
  \setbox\pgfnodeparttextbox=\hbox\bgroup #3\egroup
  \def\tikz@shape{rectangle}%
  \def\tikz@anchor{center}%
  \def\tikz@fig@name{#2}%
  \tikzset{every subnode/.try,#1}%
  \pgfpointorigin
  \tikz@scan@one@point\pgfutil@firstofone(pic cs:#2)\relax
  \advance\pgf@x by .5\wd\pgfnodeparttextbox
  \advance\pgf@y by .5\ht\pgfnodeparttextbox
  \advance\pgf@y by -.5\dp\pgfnodeparttextbox
  \pgftransformshift{}%
  \setbox\@tempboxa=\hbox\bgroup
  \pgfutil@ifundefined{pgf@sh@s@\tikz@shape}%
  {\PackageError{pgf}{Unknown shape ``\tikz@shape''}{}}%
  {%
    {%
      \let\pgf@sh@savedmacros=\pgfutil@empty% MW
      \let\pgf@sh@savedpoints=\pgfutil@empty%
      \def\pgf@sm@shape@name{\tikz@shape}% CJ % TT added prefix!
      \csname pgf@sh@s@\tikz@shape\endcsname%
      \pgf@sh@savedpoints%
      \pgf@sh@savedmacros% MW
      \pgftransformshift{%
        \pgf@sh@reanchor{\tikz@shape}{\tikz@anchor}%
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      }%
      \expandafter\pgfsavepgf@process\csname pgf@sh@sa@\tikz@fig@name\endcsname{%
       \pgf@sh@reanchor{\tikz@shape}{\tikz@anchor}% FIXME : this is double work!
      }%
      % Save the saved points and the transformation matrix
      \edef\pgf@node@name{\tikz@fig@name}%
      \ifx\pgf@node@name\pgfutil@empty%
      \else%
        \expandafter\xdef\csname pgf@sh@ns@\pgf@node@name\endcsname{\tikz@shape}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@np@\pgf@node@name\endcsname}%
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedpoints}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@ma@\pgf@node@name\endcsname}% MW
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedmacros}% MW
        \pgfgettransform\pgf@temp
        \expandafter\xdef\csname pgf@sh@nt@\pgf@node@name\endcsname{\pgf@temp}%
        \expandafter\xdef\csname pgf@sh@pi@\pgf@node@name\endcsname{\pgfpictureid}%
      \fi%
    }%
  }%
  \egroup
  \box\pgfnodeparttextbox
  \endgroup
}
\def\usetikzmarklibrary{\pgfutil@ifnextchar[{\use@tikzmarklibrary}{\use@@tikzmarklibrary}}%}
\def\use@tikzmarklibrary[#1]{\use@@tikzmarklibrary{#1}}
\def\use@@tikzmarklibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname tikzmark@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let\csname tikzmark@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tikzmark@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tikzmark@library@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \pgfutil@InputIfFileExists{tikzmarklibrary\pgf@temp.code.tex}{}{
          \PackageError{tikzmark}{I did not find the tikzmark extras library '\pgf@temp'.}{}
        }%
      \catcode`\@=\csname tikzmark@library@#1@atcode\endcsname
      \catcode`\|=\csname tikzmark@library@#1@barcode\endcsname
      \fi%
    \fi
  }%
}

%% 
%% Copyright (C) 2011-2016 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the file  tikzmark.dtx
%% and the derived files           tikzmark.ins,
%%                                 tikzmark.pdf,
%%                                 tikzlibrarytikzmark.code.tex, and
%%                                 tikzmarklibrarylistings.code.tex
%% 
%%
%% End of file `tikzlibrarytikzmark.code.tex'.


==> tikzlibrarytikzmark.code.tex <==
%%
%% This is file `tikzlibrarytikzmark.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tikzmark.dtx  (with options: `tikzlibrary')
%% ----------------------------------------------------------------
%% tikzmark --- remembering absolute positioning with TikZ.
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\tikzset{%
  remember picture with id/.style={%
    remember picture,
    overlay,
    save picture id=#1,
  },
  every picture/.append style={%
    execute at end picture={%
      \ifpgfrememberpicturepositiononpage%
      \edef\pgf@temp{%
        \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\thepage}}}%
      \pgf@temp
      \fi%
    },
  },
  save picture id/.code={%
      \protected@write\pgfutil@auxout{}{%
        \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
  },
  if picture id/.code args={#1#2#3}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#3}%
    }{
      \pgfkeysalso{#2}%
    }
  },
  next page/.is choice,
  next page vector/.initial={\pgfqpoint{0pt}{0pt}},
  next page/below/.style={%
    next page vector={\pgfqpoint{0pt}{-\the\paperheight}}%
  },
  next page/above/.style={%
    next page vector={\pgfqpoint{0pt}{\the\paperheight}}%
  },
  next page/left/.style={%
    next page vector={\pgfqpoint{-\the\paperwidth}{0pt}}%
  },
  next page/right/.style={%
    next page vector={\pgfqpoint{\the\paperwidth}{0pt}}%
  },
  next page/ignore/.style={%
    next page vector={\pgfqpoint{0pt}{0pt}}%
  },
  tikzmark prefix/.initial=,%
  tikzmark suffix/.initial=,%
}
\def\tikzmark@pp@name#1{\csname pgfk@/tikz/tikzmark prefix\endcsname#1\csname pgfk@/tikz/tikzmark suffix\endcsname}%
\def\savepointas#1#2#3#4{%
  \expandafter\gdef\csname save@pt@#1\endcsname{#2}%
  \expandafter\gdef\csname save@pt@#1@offset\endcsname{\pgfqpoint{#3}{#4}}%
}
\def\savepicturepage#1#2{%
  \expandafter\gdef\csname save@pg@#1\endcsname{#2}%
}
\def\tmk@labeldef#1,#2\@nil{%
  \edef\tmk@label{\tikzmark@pp@name{#1}}%
  \def\tmk@def{#2}%
}
\tikzdeclarecoordinatesystem{pic}{%
  \pgfutil@in@,{#1}%
  \ifpgfutil@in@%
    \tmk@labeldef#1\@nil
  \else
    \tmk@labeldef#1,(0pt,0pt)\@nil
  \fi
  \@ifundefined{save@pt@\tmk@label}{%
    \tikz@scan@one@point\pgfutil@firstofone\tmk@def
  }{%
      \pgfsys@getposition{\csname save@pt@\tmk@label\endcsname}\save@orig@pic%
      \pgfsys@getposition{\pgfpictureid}\save@this@pic%
      \pgf@process{\pgfpointorigin\save@this@pic}%
      \pgf@xa=\pgf@x
      \pgf@ya=\pgf@y
      \pgf@process{\pgfpointorigin\save@orig@pic}%
      \advance\pgf@x by -\pgf@xa
      \advance\pgf@y by -\pgf@ya
      \pgf@xa=\pgf@x
      \pgf@ya=\pgf@y
    \pgf@process{\pgfpointorigin\csname save@pt@\tmk@label @offset\endcsname}%
    \advance\pgf@xa by \pgf@x
    \advance\pgf@ya by \pgf@y
      \@ifundefined{save@pg@\csname save@pt@\tmk@label\endcsname}{}{%
        \@ifundefined{save@pg@\pgfpictureid}{}{%
          \pgfkeysvalueof{/tikz/next page vector}%
          \advance \pgf@xa by \csname save@pg@\csname save@pt@\tmk@label\endcsname\endcsname\pgf@x\relax
\advance \pgf@ya by \csname save@pg@\csname save@pt@\tmk@label\endcsname\endcsname\pgf@y\relax
          \advance \pgf@xa by -\csname save@pg@\pgfpictureid\endcsname\pgf@x\relax
\advance \pgf@ya by -\csname save@pg@\pgfpictureid\endcsname\pgf@y\relax
        }%
      }%
      \pgf@x=\pgf@xa
      \pgf@y=\pgf@ya
    \pgftransforminvert
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    }%
  }
\begingroup
\catcode`\;=\active
\gdef\tikzmark@active#1#2{%
\tikz[remember picture with id=#2] #1;}
\endgroup
\def\tikzmark@nonactive#1#2{%
\tikz[remember picture with id=#2] #1;}
\newcommand\tikzmark@outside[2][]{%
  \ifnum\catcode`\;=\active
   \let\tikzmark@next=\tikzmark@active
  \else
   \let\tikzmark@next=\tikzmark@nonactive
  \fi
  \tikzmark@next{#1}{#2}%
}
\def\tikzmark@inside#1#2{%
  \tikzset{remember picture}%
  \tikz@scan@one@point\pgfutil@firstofone#2\relax
  \protected@write\pgfutil@auxout{}{%
    \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{\the\pgf@x pt}{\the\pgf@y pt}}%
}
\def\tikzmark{%
  \ifx\pgfpictureid\@undefined
  \let\tikzmark@next=\tikzmark@outside
  \else
  \let\tikzmark@next=\tikzmark@inside
  \fi
  \tikzmark@next%
}
\newcommand\pgfmark[1]{%
    \bgroup
    \global\advance\pgf@picture@serial@count by1\relax%
    \edef\pgfpictureid{pgfid\the\pgf@picture@serial@count}%
      \pgfsys@markposition{\pgfpictureid}%
    \edef\pgf@temp{%
      \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\thepage}}}%
    \pgf@temp
    \protected@write\pgfutil@auxout{}{%
      \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
    \egroup
  }
\@ifclassloaded{beamer}{
  \renewcommand<>{\tikzmark}[2][]{\only#3{\beameroriginal{\tikzmark}[{#1}]{#2}}}
}{}
\@ifclassloaded{beamer}{
  \renewcommand<>{\pgfmark}[1]{\only#2{\beameroriginal{\pgfmark}{#1}}}
}{}
\@ifclassloaded{beamer}{
  \tikzset{
    tikzmark suffix=-\the\beamer@slideinframe
  }
}{}
\newcommand\iftikzmark[3]{%
    \@ifundefined{save@pt@#1}{%
      #3%
    }{%
      #2%
    }%
  }%
\newcommand\subnode[3][]{%
  \begingroup
  \pgfmark{#2}%
  \setbox\pgfnodeparttextbox=\hbox\bgroup #3\egroup
  \def\tikz@shape{rectangle}%
  \def\tikz@anchor{center}%
  \def\tikz@fig@name{#2}%
  \tikzset{every subnode/.try,#1}%
  \pgfpointorigin
  \tikz@scan@one@point\pgfutil@firstofone(pic cs:#2)\relax
  \advance\pgf@x by .5\wd\pgfnodeparttextbox
  \advance\pgf@y by .5\ht\pgfnodeparttextbox
  \advance\pgf@y by -.5\dp\pgfnodeparttextbox
  \pgftransformshift{}%
  \setbox\@tempboxa=\hbox\bgroup
  \pgfutil@ifundefined{pgf@sh@s@\tikz@shape}%
  {\PackageError{pgf}{Unknown shape ``\tikz@shape''}{}}%
  {%
    {%
      \let\pgf@sh@savedmacros=\pgfutil@empty% MW
      \let\pgf@sh@savedpoints=\pgfutil@empty%
      \def\pgf@sm@shape@name{\tikz@shape}% CJ % TT added prefix!
      \csname pgf@sh@s@\tikz@shape\endcsname%
      \pgf@sh@savedpoints%
      \pgf@sh@savedmacros% MW
      \pgftransformshift{%
        \pgf@sh@reanchor{\tikz@shape}{\tikz@anchor}%
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      }%
      \expandafter\pgfsavepgf@process\csname pgf@sh@sa@\tikz@fig@name\endcsname{%
       \pgf@sh@reanchor{\tikz@shape}{\tikz@anchor}% FIXME : this is double work!
      }%
      % Save the saved points and the transformation matrix
      \edef\pgf@node@name{\tikz@fig@name}%
      \ifx\pgf@node@name\pgfutil@empty%
      \else%
        \expandafter\xdef\csname pgf@sh@ns@\pgf@node@name\endcsname{\tikz@shape}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@np@\pgf@node@name\endcsname}%
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedpoints}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@ma@\pgf@node@name\endcsname}% MW
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedmacros}% MW
        \pgfgettransform\pgf@temp
        \expandafter\xdef\csname pgf@sh@nt@\pgf@node@name\endcsname{\pgf@temp}%
        \expandafter\xdef\csname pgf@sh@pi@\pgf@node@name\endcsname{\pgfpictureid}%
      \fi%
    }%
  }%
  \egroup
  \box\pgfnodeparttextbox
  \endgroup
}
\def\usetikzmarklibrary{\pgfutil@ifnextchar[{\use@tikzmarklibrary}{\use@@tikzmarklibrary}}%}
\def\use@tikzmarklibrary[#1]{\use@@tikzmarklibrary{#1}}
\def\use@@tikzmarklibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname tikzmark@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let\csname tikzmark@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tikzmark@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tikzmark@library@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \pgfutil@InputIfFileExists{tikzmarklibrary\pgf@temp.code.tex}{}{
          \PackageError{tikzmark}{I did not find the tikzmark extras library '\pgf@temp'.}{}
        }%
      \catcode`\@=\csname tikzmark@library@#1@atcode\endcsname
      \catcode`\|=\csname tikzmark@library@#1@barcode\endcsname
      \fi%
    \fi
  }%
}

%% 
%% Copyright (C) 2011-2016 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the file  tikzmark.dtx
%% and the derived files           tikzmark.ins,
%%                                 tikzmark.pdf,
%%                                 tikzlibrarytikzmark.code.tex, and
%%                                 tikzmarklibrarylistings.code.tex
%% 
%%
%% End of file `tikzlibrarytikzmark.code.tex'.

